An Equivalent Circuit Workflow for Unconstrained Optimization

We introduce a new workflow for unconstrained optimization whereby objective functions are mapped onto a physical domain to more easily design algorithms that are robust to hyperparameters and achieve fast convergence rates. Specifically, we represent optimization problems as an equivalent circuit that are then solved solely as nonlinear circuits using robust solution methods. The equivalent circuit models the trajectory of component-wise scaled gradient flow problem as the transient response of the circuit for which the steady-state coincides with a critical point of the objective function. The equivalent circuit model leverages circuit domain knowledge to methodically design new optimization algorithms that would likely not be developed without a physical model. We incorporate circuit knowledge into optimization methods by 1) enhancing the underlying circuit model for fast numerical analysis, 2) controlling the optimization trajectory by designing the nonlinear circuit components, and 3) solving for step sizes using well-known methods from the circuit simulation. We first establish the necessary conditions that the controls must fulfill for convergence. We show that existing descent algorithms can be re-derived as special cases of this approach and derive new optimization algorithms that are developed with insights from a circuit-based model. The new algorithms can be designed to be robust to hyperparameters, achieve convergence rates comparable or faster than state of the art methods, and are applicable to optimizing a variety of both convex and nonconvex problems.

==> Discussion.tex <==
\section{Discussion}
\label{sec:discussion}

The proposed equivalent circuit framework develops an analogous physical system through which we can gain insights. The methods we have discussed can be altered or replaced based on the system being optimized. Nonetheless, the equivalent circuit analogy enables an overarching framework to develop new methods which can be broadly broken down into four hierarchy sections shown in the figure below. 

\includegraphics[scale=0.3]{Figures/EC_heirarchy.png}

The basis of the framework is the equivalent circuit representation of the mathematical problem as shown in the first section of the figure. After the equivalent circuit model is developed, we can define modifications in the circuit, such as the current source stepping or adding an inductor, to reach steady-state faster. Future research can develop further modifications to the circuit to suit the application. With a circuit defined, we now are in the section that defines a solution trajectory by developing feedback control that affects the nonlinear capacitance. A method to control the nonlinear capacitors is proposed in section XX which uses a Lyapunov function related to the energy stored in the system. We can develop other control mechanisms by proposing alternative Lyapunov functions that can be specialized to a system. Nonetheless, the main idea is centered around feedback that controls the capacitance. Finally, we can solve for the trajectory numerically using a direct ODE solver that approximates the state at each time-point using a numerical integration method. In our work, we use a single time-step explicit integration method known as Forward Euler. However, we can utilize both implicit and alternative explicit methods. The concepts of local truncation error and steady-state convergence in section XX will remain relevant with alternate integration methods.

	The framework is generalized in the figure to facilitate new and existing first-order gradient-based methods. As we have shown in section XX, the equivalent circuit analogy can realize various other first order methods such as momentum-based methods and heavy-ball. 


==> Equivalent_Circuit.tex <==
\section{Equivalent Circuit and Adjoint Circuit Models}
\label{sec:equivalent-circuit}

The OT-ODE is a continuous-time realization of general first-order optimization methods which allows us to design an equivalent physical system. With the advent in circuit simulation, we choose to define an \emph{equivalent circuit} representation of the OT-ODE. This representation will be vital in developing important properties for faster convergence. Additionally, we design an adjoint circuit to the equivalent circuit model that achieves an identical trajectory but will give further insight into designing the nonlinear control for guaranteed and faster convergence.

\subsection{Equivalent Circuit Model}

\begin{definition}
An \emph{Equivalent Circuit} (EC) of the desired OT-ODE \eqref{otode} is a circuit whose transient voltage response is equal to the OT-ODE in \eqref{otode}. For $\x\in\mathbb{R}^n$, a multidimensional OT-ODE may be represented by a set of $n$ coupled sub-ECs, each representing the trajectory of one $\x_i$. 
%For an OT-ODE expressed in (XX), we can define an equivalent circuit model as a circuit whose voltage response is the same as the state OT-ODE used to solve \eqref{prob}.

\iffalse
\begin{figure}[h]
    \centering
    \includegraphics[]{Figures/EC_single_circuit.png}
    \caption{Equivalent Sub-Circuit for a single variable in the OT-ODE}
    \label{fig:EC}
\end{figure}
\fi
\begin{figure}[h!]
    \centering
    \begin{circuitikz} \draw
    (0,0) to[C=$Z_{ii}(\x(t))$] (0,3)
      to[short] (3,3)
      to[cI, l=$f_i(\x(t))$] (3,0)
      to[short] (0,0)
    ;
    \draw (3,3) to [short,-o] (4,3) node[above]{$\x_i(t)$};
    \draw (1.5,0) node[ground] (){};
    \end{circuitikz}
    \caption{Equivalent Circuit}
    \label{fig:ECorig}
\end{figure}
\end{definition}

The sub-circuit in Figure \ref{fig:ECorig} is a physical representation of the transient waveform of a single variable, $\x_i$ in the OT-ODE. Each sub-EC model is composed of two circuit elements: a nonlinear capacitor and a voltage-controlled current source (VCCS). The voltage across the capacitor, $\x_i(t)$, represents the trajectory of a single state-variable.  Furthermore, the current produced by the VCCS, $f_i(\x)$ on the right is equal to the gradient of the objective, $\nabla_x f_i$



The OT-ODE is rederived using the EC model by solving Nodal-Analysis \cite{pillage1995electronic}. Nodal-analysis is a formal method that characterizes Kirchhoff’s Current Law (KCL) at each node. KCL is a physical law stating that the sum of currents entering a node must equal the sum of currents leaving. Applying KCL to each sub-EC, as shown in Figure \ref{fig:EC}, we see the currents leaving node of the sub-circuit are the current from the non-linear capacitor, $I_c(x(t))$ and the voltage-controlled current source, $f(X(t))$. Accordingly, Nodal-analysis produces the following expression which i identical to the OT-ODE:

\begin{equation}
    Z_{ii}(\x(t))\dot{\x} + \nabla_xf_{i}(\x(t)) = 0
\end{equation}

The EC model provides insights to the physical behavior of the circuit  which will provide intuition for the control and convergence of the OT-ODE. 

\subsubsection{Capacitor in EC Model}
The nonlinear capacitor, shown in red in Figure \ref{fig:EC} provides a transient current through the circuit, $I_c$.
\begin{definition}
The current-voltage relationship of the nonlinear capacitor can be described as
\begin{equation}
    I_{C_i} = Z_{ii}(\x(t))\dot{\x_i}(t)
    \label{eq:cap_eq}
\end{equation}
where $Z_{ii}(\x(t))$ is the nonlinear capacitance that is a function of the state variables, $\x$. In the entire EC-model, the capacitance matrix, $Z(\x(t))$ is a diagonal matrix (with diagonal entries of $Z_{ii}$) representing a nonlinear capacitor to ground at each node. The relative value of the capacitance between each sub-circuit provides a change in trajectory of the overall optimization. 
\end{definition}


Initially ($\forall t<0$), the voltage across the capacitor is held at the initial condition of $x_i(t<0)=x_i_{0}$. After $t=0$, the capacitor is no longer held at the voltage and charges/discharges according to the transient response \eqref{eq:cap_eq}
%Initially, the capacitor is charged with a charge, $Q_o$, with a fixed voltage of $x_0$ for all $t<0$. After $t=0$, the charge on the capacitor changes to
Eventually, the EC model reaches a steady-state ($t>t_{ss}$), at which the voltage across the capacitor is unchanging. At the steady-state condition, the capacitor current will equal 0, as $\dot{\x}_i=0$ and therefore be at an equilibrium. In this state, the capacitor is no longer charging or discharging and has reached an equilibrium with the rest of the system.

In this work we design $Z(\x(t))$ to provide fast convergence to steady-state using intuition from the energy stored in the capacitor.

\iffalse
\begin{definition}

The nonlinear capacitor, with $Z_{ii}>0$ is a passive, energy storage device that stores and releases available energy. The \emph{energy in the nonlinear capacitor}, $E_{C_i}$, is described as
\begin{equation}
    E_{C_i}(t)=\frac{1}{2}Z_{ii}(\x)\x^2(t)
\end{equation}

\end{definition}
It is apparent from the EC model that the energy in the capacitor is transferred to the element on the right (the voltage controlled current source) and at steady-state, the energy stored will remain constant.
\fi

\subsubsection{Voltage-Controlled Currrent Source}

The last component of the EC model is the VCCS as shown in blue in Figure \ref{fig:EC}, which captures the gradient information of the original objective. The VCCS achieves this by producing a current equal to the gradient of the objective as a function of the voltages in the EC system, $\x$. 

At steady-state, the capacitor current is equal to 0 and applying KCL to the EC in Figure \ref{fig:EC}, implies that the current from the VCCS must also equal zero. Therefore, at steady-state the EC has reached a point where $f(\x)=\nabla_\x F(\x)=0$. This implies that the steady-state of the EC model is achieved when $f(\x)=\nabla_\x F(\x)=0$, which is a necessary condition for reaching a critical point in the original objective.

\subsection{Adjoint Circuit Model}

To gain further insight into the energy stored in the capacitor, we construct a time-derivative version of the OT-ODE as described by:


\begin{equation}
    \frac{d}{dt}(\Zeta(\x(t))\dot{\x}(t)) = - \dot{f}(\x(t)) \;\;\; \dot{x}(0) = \dot{x_0}
\end{equation}
The time-derivative equation is vital for analyzing the convergence properties of the original OT-ODE. Importantly, the time-derivative OT-ODE has an identical trajectory of $\x$ compared to the original OT-ODE in \ref{otode}. 

    \begin{lemma}
 The trajectory of $\x$ inn the time-derivative OT-ODE is identical to the trajectory of $\x$ in the OT-ODE given that $Z(\x(t))$ is continuous.

    \textbf{Proof:} I dunno

    \end{lemma}



To gain insight into the trajectory of $\x$, we construct an equivalent circuit model for the time-derivative OT-ODE as shown below:

\begin{figure}[h]
    \centering
    \begin{circuitikz} \draw
    (0,0) to[C, i^<=$(\nabla_t Z(\x(t))\dot\x_i(t))_i$] (0,3)
      to[short] (3,3)
      to[cI, l=$\dot{f}_i(\x(t))$] (3,0)
      to[short] (0,0)
    ;
    \draw (3,3) to [short,-o] (4,3) node[above]{$\dot\x_i(t)$};
    \draw (1.5,0) node[ground] (){};
    \end{circuitikz}
    \caption{Adjoint Equivalent Circuit}
    \label{fig:ECadj}
\end{figure}

This new equivalent circuit model is an \emph{adjoint} circuit to the EC model in Figure \ref{fig:EC} that now represents $\dot{\x}(t)$ as the node voltage of each adjoint sub-EC.
The steady-state of the adjoint EC model now coincides with $\dot{\x}=0$, which means the node voltage is zero. 

We can treat the adjoint EC model as a zero-input circuit, with no active sources, and a natural unforced steady-state at $\dot{\x}=0$. In general, the energy initially stored in a zero-input circuit dissipates through  passive elements until there is no stored energy left in the circuit. Understanding this behavior provides intuition on the overall trajectory of the state variables.


Similar to the EC model, the adjoint circuit is composed of two elements, namely a capacitor model and a VCCS.


\subsubsection{Adjoint Circuit Capacitor}

The capacitor in the adjoint circuit produces a current that is a function of the node voltage of the adjoint sub-circuit, $\dot{x}(t)$. The current $\bar{I}_c(t)$ is defined by:
\begin{equation}
    \bar{I}_c(t) = \frac{d}{dt}(\Zeta(\x(t))\dot{x}(t))
\end{equation}
Understanding that current is the time-derivative of charge, we can also conclude that the amount of charge stored in the adjoint capacitor, $\bar{Q}_c(t)$ can be defined as:
\begin{equation}
    \bar{Q}_c(t) = \Zeta(\x(t))\dot{x}(t)
\end{equation}

The capacitor in the adjoint circuit stores energy in its electric field. The total energy stored in the adjoint circuit can be described as

\begin{equation}
    \bar{E}_c(t) = \frac{\bar{Q}_{C}^2(t)}{2\Zeta(\x(t))}
\end{equation}

The energy stored in the adjoint capacitor is proportional to the square of charge stored ($\bar{Q}_{C}^2(t)$). As the adjoint circuit has a natural steady-state at $\dot{x}=0$, the charge naturally will dissipate through the transient response and tt steady-state, the adjoint capacitors will no longer have any charge, $\bar{Q}_c=0$. This also means the stored energy in the adjoint circuit, $\bar{E}_C(t)$ goes to zero. In this respect, the energy initially stored in the adjoint capacitors ($\bar{E}_c(0)$) must dissipate throughout the rest of the adjoint circuit (the VCCS elements). 


\subsubsection{Adjoint VCCS Model}

The currrent produced by the VCCS elements in the adjoint circuit represent the time-derivative of the gradient, with the current equal to:
\begin{equation}
    \bar{I}_f(t) = \dot{f}(\x(t))
\end{equation}
Using the chain rule, the current can also be described as :
\begin{equation}
    \bar{I}_f(t) = \frac{d f}{dx}\dot{x}(t)
\end{equation}
which now represents a nonlinear conductance equal to $\frac{d f}{d \x}$.


As described earlier, the adjoint circuit is a zero-input circuit that should ideally dissipate the initial energy stored in the adjoint capacitors.  Through the circuit interpretation, the only elements capable of dissipating the energy are the adjoint VCCS elements. 


If the adjoint VCCS elements are capable of \emph{always} dissipating energy, then through the circuit interpretation, the  energy initially stored in the adjoint circuit will dissipate and the system converge to a zero-energy steady-state. 
Our goal is to design a method to ensure the VCCS elements dissipate energy at all times. One way to achieve this is by ensuring the VCCS elements are \emph{passive}. 

\begin{definition}
Passive circuit elements do not generate energy, but rather dissipate, store or release energy. 

A passive, non-storage element can be further defined as an element whose power consumption is always greater than 0. A non-storage element with a voltage potential of $v$ and a current $i$ is passive if and only if:
\begin{equation}
    vi\geq 0
\end{equation}
\end{definition}

The passivity condition for the adjoint VCCS elements would be:
\begin{equation}
    \frac{d f_i(\x_i)}{d t} \dot{\x}_i \geq 0
\end{equation}

Along with the passive adjoint capacitors (with $Z_{ii}>0$ and only store and release energy), if all the components of the adjoint circuit are passive, then we can conclude that the entire adjoint EC is a passive circuit. 
 


\begin{definition}
A passive \emph{circuit} is one that always dissipates the amount of stored energy in the circuit. Given a circuit at time $t$ with energy stored, $E(t)$, the condition for passivity is:
\begin{equation}
    E(t+T) \leq E(t) \forall t,T
\end{equation}
Importantly, if a circuit is composed solely of passive elements, then it is passive. 

\end{definition}




\begin{comment}
The response of the VCCS can be described as the sum of a homogenous term, $f_h$, and a particular term, $f_p$:
\begin{equation}
    f(X(t))=f_h(X(t))+f_{p}(X(t)),
\end{equation}

where the homogeneous component of the VCCS satisfies the property,
\begin{equation*}
    f_h(X(t))=0 \Longleftrightarrow X=0.
\end{equation*}

This separation aids in developing a homogeneous version of the OT-ODE, and is in line with general ODE methodology. %The homogeneous version of the OT-ODE will be vital in developing heuristics for trajectory control.

%This condition will allow us to define the solution of the homogeneous version of the OT-ODE as $X=0$.

Without loss of generality, we can also shift the state variables by a known vector, such as the initial conditions, $X_0$ to define an adjoint system:
\begin{equation}
    \dot{\Bar{X}}(t)=-f(\Bar{X}(t)+X_0)
\end{equation}
where $\bar{X}(t)=X(t)-X_0$. The trajectory of the adjoint system above is identical to the trajectory of the original OT-ODE.\todo{do we need this discussion? If so, motivate why}

To specify $\fnh$ and $\fh$, the particular term must first be extracted:
\begin{align*}
    f(0)&=\fh(0)+\fnh(0) = \fnh(0)\Rightarrow \fnh(\x(t))=f(0)=I_x.
\end{align*}

The homogeneous component is therefore, 
\begin{equation*}
    f_h(X)=f(X)-I_X.
\end{equation*}

Note that the particular component is constant through time, and therefore can be represented as a constant current source, $I_X$. The EC drawn with respect to $\fnh$ and $\fh$ is shown in Figure \ref{fig:EC2}.%A constant current source is an active element that can provide energy. 

\begin{figure}
    \centering
    \includegraphics[]{Figures/EC_single_circuit_split.png}
    \caption{Caption}
    \label{fig:EC2}
\end{figure}


Importantly, the homogeneous component is a voltage-controlled voltage source that may be active, or passive based on the gradient information. The amount of power a single homogeneous VCCS component, $f_h_i (X(t))$ absorbs or dissipates is equal to:   
\begin{equation}
    P_{fh_i}(t)=X_i(t)f_h_i(X(t))
\end{equation}
The separation of the particular term provides an intuitive insight that the driving source in the circuit is the constant current source, $I_X$. This element represents a constant value in the gradient or equivalently, a linear term in the objective, which drives the solution away from the trivial solution of $X=0$.
\end{comment}
At steady-state, the VCCS, $f(X)$, provides no current, indicating we have reached a local minima. 

The intuition of the circuit elements helps develop a control scheme for the non-linear capacitance, $Z(\x(t))$ based on the concepts of circuit energy and passivity.
%With the EC model separated into the homogeneous and particular components, we can now numerically solve for the trajectory of X(t) to steady-state using the following ODE that describes the system in Figure XX.
%\begin{equation}
%    Z(X(t))\dot{X}(t)=-(f_h(X(t))+I_X)
%\end{equation}
%Using a numerical integration technique, we can march through time in discrete time-steps to accurately determine the trajectory of $X$. \todo{do we need to introduce integration at this point?}
%\begin{equation}
%    X(t+\Delta t)=X(t)+\Delta t\int_t^{t+\Delta t}-Z^{-1}(X(t))(f_h(X(t))+I_X) dt
%\end{equation}
%The integral in the equation above can be approximated using various numerical integration techniques [XX] for the discrete step in time, $\Delta t$. 


\iffalse
- change X to $\x$
- make it Z = gamma^{-1}
- add a definition for circuit (6), put a lemma or theorem saying they are the same and equilibrium is equivalent
- equation (9), dont do nh, do either p (for particular) or h bar or be consistent with g (khalil)
- Equation (15) make the i a superscript or say for each component 
\fi








==> Extensions.tex <==
\section{Extending the Equivalent Circuit Model}
\label{sec:extensions}



The equivalent circuit for first-order gradient methods offers a physically intuitive framework for developing direction vectors and step-sizes. We can further utilize the circuit analogy by modifying the underlying equivalent circuit to reach steady-state faster or modifying the discretization to rederive existing optimization methods. 

\subsection{Circuit-Driven Homotopy Analysis}
Circuit simulation often uses homotopy analyses to develop fast steady-state convergence methods. A homotopy method is an iterative transformation of the network that embeds a scalar homotopy parameter, $\gamma∈[0,1]$, into the system of equations. The homotopy parameter deforms the system to define a new trajectory, controlled by $\gamma$, starting from a  relaxed, easy to solve network with a trivial solution, to the original network. 


Consider solving a general system of nonlinear equations, represented by $G(y)=0$. A homotopy method defines a simpler (often convex transformation) of the original problem denoted as $E(y)=0$. Therefore the homotopy method defines a trajectory in the solution space, guided by the scalar homotopy factor, $\gamma$, that transforms the problem from trivial problem $E(y)=0$ to the original $G(y)=0$. This process is captured by solving a new series of nonlinear equations, $H(y,\gamma)$ defined as:
\begin{equation}
    H(y,\gamma) = (1-\gamma)G(y) + \gamma E(y)=0 \;\;\; \gamma=1\xrightarrow{}0
\end{equation}

The homotopy method decrements the homotopy factor, $\gamma$, from 1 to 0 in small increments of $\Delta \gamma$. At each sub-problem, defined as $H(y,\gamma^k)=0$, the initial value of $y$ is the solution of the previous sub-problem $H(y,\gamma^k-\Delta \gamma)=0$. The homotopy method exploits fast convergence between sub-problems for fast convergence to the original problem.


There are numerous methods to embed the homotopy parameter into a system of equations and it is often difficult to choose a single embedding that offers better convergence. Circuit simulation methods have successfully relied on physical intuition to embed the homotopy parameter into their system. 


We apply a homotopy method, called source-stepping, that embeds the homotopy factor in an intuitive manner into the equivalent circuit model. This provides an intuitive methodology that iteratively transforms the optimization problem for fast convergence.

\subsubsection{ Source-Stepping Method}

The equivalent circuit model is a representation of the OT-ODE with an initial value of $x(t=0)=x_0$. The initial-value of $\x=x_0 \;\; \forall t\leq 0$ can be represented in the circuit analogy as a voltage source (with voltage $\x_0$) in parallel with each EC sub-circuit with a switch that is opened at $t=0$. The circuit representation is shown in the figure below.


To ensure the voltage remain constant for $t\leq0$, the voltage source is producing a current equal to $-f(\x_0)$. This ensures that there is zero current produced by the capacitor, thereby ensuring the voltage at the node is constant at $\x_0$. Using the principles of substitution theorem [XX], we can replace the voltage source by a current source that produces a current of $-f(\x_0)$. 



The current-stepping homotopy method embeds the scalar homotopy factor by multiplying it with the current source shown below. Rather than opening the switch at $t=0$, the homotopy method decrements the current source value to 0. The modified problem can be expressed as:

\begin{equation}
    Z(\x)\dot{\x(t)} = -f(\x(t)) + \gamma f(\x_0)
\end{equation}

At each sub-problem defined by $\gamma^k$, the modified ODE is driven to steady-state from the initial condition equal to the steady-state of the previous homotopy iteration. Intuitively, we are letting the circuit reach an intermediate steady-state before decreasing the value of the current source.

Knowing that the steady-state is bounded within a small radius of the previous steady-state, we can now take larger time-steps to reach the steady-state of each intermediate problem. This ultimately means, we can use a smaller tolerance for the local truncation error check in Algorithm XX, and instead rely on the steady-state check to ensure descent. The full algorithm for the source-stepping is shown below



\begin{comment}

\begin{definition}
Let $F(X)=0$ be  the original problem we are solving for. In our case, we define $F(X)$ as
\begin{equation}
    F(X)=Z(X)\dot{X}+f(X)=0
\end{equation}
We now introduce a modified set of equations,$H(X,\gamma)=0$, which embeds the homotopy factor into the original system as::
\begin{equation}
    H(X,\gamma)=F(X,\gamma) + G(X,\gamma)
\end{equation}

Where $F(X,1)$ is the original system of equations and $G(X)$ is the modification added onto the problem.
\end{definition}

There are numerous methods to embed the homotopy parameter into a system of equations and it is often difficult to choose a single embedding that offers better convergence. Circuit simulation methods have successfully relied on physical intuition to embed the homotopy parameter into their system.  In the source-stepping method, the homotopy method is embedded into the system by multiplying constant current sources by the homotopy parameter as shown in the figure below. In doing so, at a homotopy factor $\gamma=0$, the sources are removed, thereby leading to a trivial network with no excitation devices. By slowly incrementing the homotopy factor, the source-stepping method exploits local convergence properties by using the previous iteration homotopy solution as an initial guess. In doing so, they are able to take large step-sizes between successive homotopy problems, to reach the solution of the original problem much faster.
We employ the source-stepping method in the equivalent circuit model by multiplying the constant current source, $I_X$ with a homotopy parameter γ. This defines a series of ODEs, each with its own steady-state, as defined by:
\begin{equation}
    H(X,t,\gamma) = Z(X)\dot(X)+f_{h}(X) + \gamma I_X=0
\end{equation}

We see that the initial homotopy problem of $\gamma=0$, is a trivial problem with no excitation in the system and a easy realizable solution of $X=0$, as we have defined $f_h (X)$. For each successive homotopy problem, the initial condition is the steady-state of the previous homotopy problem. This exploits the small perturbation of the current source which ensures that our solution is within a small radius given a valid Lyapunov function. This is realized using the following theorem as derived in [XX]:

\begin{theorem}
Let the steady-state solution to a previos homotopy problem, given by $H(X,t,\gamma^k)=0$ be $X=X^k*$. 

Now suppose we are solving the successive homotopy problem given by:
\begin{equation}
    H(X,t,\gamma^{k+1})=0
\end{equation}
where $\gamma^{k+1} = \gamma^k + \Delta \gamma$. $\Delta \gamma$ represents an increment in the homotopy factor.
\end{theorem}

\begin{definition}

We now can define the following homotopy problem for the source-stepping homotopy method as:
\begin{align}
   H(X,t,\gamma^{k+1})= Z(X)\dot(X(t)) + f_h(X) + \gamma^{k+1}I_X=0 \\
   X(0) = X^{k*}
\end{align}

We can seperate the problem above further as:
\begin{align}
   H(X,t,\gamma^{k+1})= Z(X)\dot(X(t)) + f_h(X) + (\gamma^{k}+\Delta \gamma)I_X=0 \\
    X(0) = X^{k*} \\
    => H(X,t,\gamma^{k+1})= H(X,t,\gamma^{k}) + \Delta \gamma I_X=0 \\
    X(0) = X^{k*}
\end{align}

We can view the added constant term, $\Delta \gamma I_X$, as a perturbation to the system, $H(X,t,\gamma^k)$, at steady-state.
\end{definition}


Knowing from section XX, that $H(X,t,\gamma^k)$ is a stable system with a valid Lyapunov function, we can now define a bound for the effect of the perturbation on the state. 

\begin{theorem}

Let a stable system at steady-state, $F_1(X,\dot{X},t)=0$, have  a valid Lyanpuv function, $V_1(X,t)$. We can perturb the system with a vector, $\eta \in R^n$:
\begin{equation}
    F_1(X,\dot{X},t)+\eta=0
\end{equation}
Assuming the perturbation is bounded
\begin{equation}
    \|\eta \| \leq \delta
\end{equation}
then the state of the perturbed system is bounded by
\begin{equation}
    \|X\| \leq e^{something} + \beta \delta
\end{equation}

\end{theorem}
The proof for the theorem above is given in [XX].

\end{comment}

%Knowing that the solution is bounded within a small radius, we can now take larger time-steps to reach the steady-state of each intermediate problem. This ultimately means, we can use a smaller tolerance for the local truncation error check in Algorithm XX, and instead rely on the steady-state check to ensure descent. The full algorithm for the source-stepping is shown below


\begin{algorithm}
\caption{Source-Stepping Algorithm}
\begin{algorithmic}[2]
\Procedure{Source-Stepping}{$\Delta \gamma$, F(\cdot), X_0}
\State \gamma = 0
\State X^{k*} = X_0
\While{\gamma <1}
\State Solve to steady-state: \\ Z(X)\dot(X) = -f_h(X) -\gamma I_X \\
X(0) = X^{k*} 
\State Set X^{k*} = X(t_{ss}) 
\State \gamma += \Delta \gamma
\EndWhile


\end{algorithmic}
\end{algorithm}


In the context of optimization, we have defined a homotopy method embedded into the original objective function, $F(X)$ by adding a linear term of $\x \nabla f(\x_0)$ in the objective. The added term is iteratively reduced and is essentially a form of contour stepping, in which we iteratively modify a portion of the objective to gain robust and timely convergence. However, we could only develop this intuition through the equivalent circuit framework by understanding that the constant current source can be ramped up in steps. In the results section, we highlight the efficacy of this approach especially on nonconvex problems.




==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{An Equivalent Circuit Workflow for Unconstrained Optimization}{D. Doe, P. T. Frank, and J. E. Smith}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{An Equivalent Circuit Workflow for Unconstrained Optimization}

\iffalse
% Authors: full names plus addresses.
\author{Aayushya Agarwal\thanks{Dept. of Electrical and Computer Engineering at
Carnegie Mellon University, Pittsburgh, PA 
  (\email{ aayushya, cfiscko, pileggi,soummyak@andrew.cmu.edu}).}
\and Carmel Fiscko \footnotemark[1]
\and Larry Pileggi\footnotemark[1] 
\and Soummya Kar \foornotemark[1] 
\and Bruno Sinopoli \thanks{ Dept. of Electrical and Systems Engineering at Washington University in St. Louis, MO at 1 Brookings
Dr, St. Louis, MO 63130. bsinopoli@wustl.edu}}
\fi
\author{Dianne Doe\thanks{Imagination Corp., Chicago, IL 
  (\email{ddoe@imag.com}, \url{http://www.imag.com/\string~ddoe/}).}
\and Paul T. Frank\thanks{Department of Applied Mathematics, Fictional University, Boise, ID 
  (\email{ptfrank@fictional.edu}, \email{jesmith@fictional.edu}).}
\and Jane E. Smith\footnotemark[3]}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

